Modelling and Analysis of Biochemical Signalling Pathway Cross-talk

Signalling pathways are abstractions that help life scientists structure the coordination of cellular activity. Cross-talk between pathways accounts for many of the complex behaviours exhibited by signalling pathways and is often critical in producing the correct signal-response relationship. Formal models of signalling pathways and cross-talk in particular can aid understanding and drive experimentation. We define an approach to modelling based on the concept that a pathway is the (synchronising) parallel composition of instances of generic modules (with internal and external labels). Pathways are then composed by (synchronising) parallel composition and renaming; different types of cross-talk result from different combinations of synchronisation and renaming. We define a number of generic modules in PRISM and five types of cross-talk: signal flow, substrate availability, receptor function, gene expression and intracellular communication. We show that Continuous Stochastic Logic properties can both detect and distinguish the types of cross-talk. The approach is illustrated with small examples and an analysis of the cross-talk between the TGF-b/BMP, WNT and MAPK pathways.

==> eptcsdata.tex <==
\providecommand{\event}{E. Merelli and P. Quaglia (Eds.)\\
From Biology To Concurrency and back 2010 (FBTC'10)
}
\providecommand{\volume}{19}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{40}
\providecommand{\eid}{3}

